HetPipe: Enabling Large DNN Training on (Whimpy) Heterogeneous GPU Clusters through Integration of Pipelined Model Parallelism and Data Parallelism

Deep Neural Network (DNN) models have continuously been growing in size in order to improve the accuracy and quality of the models. Moreover, for training of large DNN models, the use of heterogeneous GPUs is inevitable due to the short release cycle of new GPU architectures. In this paper, we investigate how to enable training of large DNN models on a heterogeneous GPU cluster that possibly includes whimpy GPUs that, as a standalone, could not be used for training. We present a DNN training system, HetPipe (Heterogeneous Pipeline), that integrates pipelined model parallelism (PMP) with data parallelism (DP). In HetPipe, a group of multiple GPUs, called a virtual worker, processes minibatches in a pipelined manner, and multiple such virtual workers employ data parallelism for higher performance. We also propose a novel parameter synchronization model, which we refer to as Wave Synchronous Parallel (WSP) to accommodate both PMP and DP for virtual workers, and provide convergence proof of WSP. Our experimental results on a given heterogeneous setting show that with HetPipe, DNN models converge up to 49% faster compared to the state-of-the-art DP technique.

==> anal_backup.tex <==
\section{Introduction}
\begin{proof}
    Since $f_t$ are convex
\begin{equation}
    TR[W] \leq \sum_{t=1}^T \left\langle \nabla f_t\left(\Tilde{w}_t\right), \tilde{w}_t - w^* \right\rangle = \sum_{t=1}^T \left\langle \tilde{g}_t, \tilde{w}_t - w^* \right\rangle,
\end{equation}
where $\tilde{g}_t \coloneqq \nabla f_t(\tilde{w}_t)$.
\begin{lemma} \textit{(This is Lemma 2 in the paper)}
    For all $w^* \in \mathbb{R}^n$ and $t > 0$,
    \begin{multline}
        \left\langle \tilde{w}_t - w^*, \tilde{g}_t \right\rangle = \frac{\eta_t}{2} \Vert \tilde{g}_t \Vert^2 + \frac{D\left(w^* \Vert w_{t+1}\right) - D\left(w^* \Vert w_{t}\right)}{\eta_t} \\
        + \left[\sum_{i \in \mathcal{R}_t} \eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle - \sum_{i \in \mathcal{Q}_i} \eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle\right].
    \end{multline}
\end{lemma}
\begin{proof} We have
    \begin{multline}
    D\left(w^* \Vert w_{t+1}\right) - D\left(w^* \Vert w_{t}\right) = \frac{1}{2} \eta_t^2 \left\Vert \tilde{g}_t \right\Vert^2 - \eta_t \left\langle \tilde{w}_t - w^*, \tilde{g}_t \right\rangle \\
    - \eta_t \left\langle w_t - \tilde{w}_t, \tilde{g}_t \right\rangle,
\end{multline}
with the last term is
\begin{equation}
    \left\langle w_t - \tilde{w}_t, \tilde{g}_t \right\rangle = - \sum_{i \in \mathcal{R}_t}\eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle + \sum_{i \in \mathcal{Q}_t} \eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle.
\end{equation}
Therefore,
\begin{multline}
    \left\langle \tilde{w}_t - w^*, \tilde{g}_t \right\rangle = \frac{\eta_t}{2} \Vert \tilde{g}_t \Vert^2 + \frac{D\left(w^* \Vert w_{t+1}\right) - D\left(w^* \Vert w_{t}\right)}{\eta_t} \\
    + \left[\sum_{i \in \mathcal{R}_t}\eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle - \sum_{i \in \mathcal{Q}_t} \eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle\right].
\end{multline}
\end{proof}
We use Lemma 2 to find the upper bound of the regret $R[W]$:
\begin{align}
    \sum_{t = 1}^T \frac{\eta_t}{2} \Vert \tilde{g}_t \Vert^2 & \leq \sum_{t = 1}^T \frac{\eta_t}{2} L^2 \nonumber \\
    & = \frac{1}{2}\sum_{t = 1}^T \frac{\sigma}{\sqrt{t}} L^2 \leq \sigma L^2 \sqrt{T},
\end{align}
and
\begin{align}
    & \sum_{t = 1}^T \frac{D\left(w^* \Vert w_{t+1}\right) - D\left(w^* \Vert w_{t}\right)}{\eta_t} \notag \\
    = \quad & \frac{D(w^* \Vert w_1)}{\eta_1} - \frac{D(x^* \Vert w_{T+1})}{\eta_t} + \sum_{t=2}^{T}\left[D(w^* \Vert w_t) \left(\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}} \right)\right] \notag \\
    \leq \quad & \frac{M^2}{\sigma} + 0 + \frac{M^2}{\sigma} \sum_{t=2}^T \left[\sqrt{t} - \sqrt{t - 1}\right] \notag \\
    = \quad & \frac{M^2}{\sigma} + \frac{M^2}{\sigma}\left[\sqrt{T} - 1\right] \notag \\
    = \quad & \frac{M^2}{\sigma}\sqrt{T},
\end{align}
and
\begin{align}
    & \sum_{t = 1}^T \left[\sum_{i \in \mathcal{R}_t}\eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle - \sum_{i \in \mathcal{Q}_t} \eta_i \left\langle \tilde{g}_i, \tilde{g}_t \right\rangle\right] \nonumber \\
    \leq \quad & \sum_{t = 1}^T \left(\left\vert \mathcal{R}_t \right\vert + \left\vert \mathcal{Q}_t \right\vert\right) \eta_{\max(1, t - F_s - s_gN)} L^2 \nonumber \\
    = \quad & L^2 \left[\sum_{t=1}^{F_s + s_gN} \left(\left\vert \mathcal{R}_t \right\vert + \left\vert \mathcal{Q}_t \right\vert\right) \eta_1 \right. \nonumber \\
    & \qquad + \left. \sum_{t=F_s + s_gN + 1}^T \left(\left\vert \mathcal{R}_t \right\vert + \left\vert \mathcal{Q}_t \right\vert\right) \eta_{t - F_s - s_gN}\right] \nonumber \\
    = \quad & L^2 \left[\sum_{t=1}^{F_s + s_gN} \left(\left\vert \mathcal{R}_t \right\vert + \left\vert \mathcal{Q}_t \right\vert\right) \sigma \right. \nonumber \\
    & \qquad + \left. \sum_{t=F_s + s_gN + 1}^T \left(\left\vert \mathcal{R}_t \right\vert + \left\vert \mathcal{Q}_t \right\vert\right) \frac{\sigma}{\sqrt{t - F_s - s_gN}}\right] \nonumber \\
    \leq \quad & \sigma L^2 (2s_g + s_l)(N - 1) \left[F_s + s_gN + \sum_{t=F_s + s_gN + 1}^T \frac{1}{\sqrt{t - F_s - s_gN}}\right] \nonumber \\
    \leq \quad & \sigma L^2 (2s_g + s_l)N \left[F_s + s_gN + 2\sqrt{T - F_s - s_gN}\right] \nonumber \\
    \leq \quad & \sigma L^2 (2s_g + s_l)N \left(F_s + s_gN\right) + 2 \sigma L^2 (2s_g + s_l)N \sqrt{T} \nonumber \\ 
    \leq \quad & \sigma L^2 (2s_g + s_l)(s_g + Fs_l)N^2 + 2 \sigma L^2 (2s_g + s_l)N \sqrt{T}
\end{align}
Therefore,
\begin{multline}
    TR[W] \leq \sigma L^2 \sqrt{T} + \frac{M^2}{\sigma}\sqrt{T} + \sigma L^2 (2s_g + s_l)(s_g + Fs_l)N^2 \\ 
    + 2 \sigma L^2 (2s_g + s_l)N \sqrt{T}
\end{multline}
Let the initial $\sigma = \frac{M}{L\sqrt{(2s_g + s_l)N}}$, then
\begin{align}
    TR[W] & \leq \frac{ML\sqrt{T}}{\sqrt{(2s_g + s_l)N}} + ML\sqrt{(2s_g + s_l)NT} \notag \\
    & \quad + ML(s_g + Fs_l)N\sqrt{(2s_g + s_l)N} + 2ML \sqrt{(2s_g + s_l)NT} \nonumber \\
    & = ML \sqrt{(2s_g + s_l)NT} \left[\frac{1}{(2s_g + s_l)N} + 1 + \frac{(s_g + Fs_l)N}{\sqrt{T}} + 2\right].
\end{align}
We have $\frac{1}{(2s_g + s_l)N} + \frac{(s_g + Fs_l)N}{\sqrt{T}} \leq 1$ when $T$ is large enough. Therefore we get
\begin{equation}
    TR[W] \leq 4ML\sqrt{(2s_g + s_l)NT},
\end{equation}
or
\begin{equation}
    R[W] \leq 4ML\sqrt{\frac{(2s_g + s_l)N}{T}}
\end{equation}
\end{proof}

==> implementation_scheduling.tex <==
\jay {\\
pipelining 실행을 위해 VW는 하나의 모델에 대해서 n개의 thread를 실행 \\
각 thread는 minibatch의 순서대로 실행 \\
각 파티션에서 어떤 thread를 실행할지에 대한 scheduling이 필요 \\
\begin{itemize}
\item 파티션에서 실행할 thread를 scheduling 하기 위해 텐서플로우에서 scheduler operation을 만듦
\item scheduler operation은 tensorflow의 placeholder로 실행 정보를 파라미터로 받음 (virtual worker index, partition index, minibatch number)
\item operation은 scheduling을 수행하며 input tensor를 output tensor로 그대로 보냄
\item scheduler operation은 pipe\_scheduler\_start\_op과 pipe\_scheduler\_end\_op의 두 종류가 있고 각 파티션의 시작과 끝에 위치
\item pipe\_scheduler\_start\_op의 동작 \\
\quad (1) 파티션 큐 (실제 구현 자료구조는 list)에 실행 정보 등록 \\
\quad - 실행 정보는 forward/backward 정보와, minibatch 번호의 pair로 구성 (i.e.  <fwd, 8>, <bwd, 7>, <fwd, 9>) \\
\quad (2) 스케줄링 \\
\qquad - forward와 backward가 있을 때 backward가 우선순위 높음 \\
\qquad - minibatch의 낮은 번호가 우선순위 높음 \\ 
\quad (3-1) 스케줄링 되지 않으면 wait - 이후 notify로 깨워지면 다시 (2) 스케줄링부터 시작 \\
\quad (3-2) 스케줄링 되면 해당 파티션의 running state = True로 하고 실행
\item pipe\_scheduler\_end\_op 동작 \\
\quad 파티션의 끝에서 해당 파티션의 실행이 끝났음을 파티션 큐의 thread에게 알림 \\
\quad - 실행 정보 (i.e. <bwd, 7>) 를 파티션 큐에서 제거 \\
\quad - running state \= False로 변경 \\
\quad - 해당 파티션에서 wait 중인 thread를 notify하여 깨워주기 \\
\end{itemize}  
forward pass의 파티션과 backward pass의 파티션 모두 같은 방식으로 동작, 
virtual worker가 여러 개일 때에도 virtual worker 별로 동작 
}

==> implementation_w_mgr.tex <==
\gc {\\
\begin{itemize}
\item weight management implementation \\
\quad - Tensorflow python API, python threading API를 사용하여 구현 \\
\\
\item local weight management \\
\quad - weight(parameter) versioning을 위해 virtual worker 내의 thread 별로 Tensorflow model graph와 weight를 각각 정의. (이하 local weight이라 지칭). Tensorflow 'variable\_scope' 를 사용하여 각 thread가 각자의 weight와 graph에만 연산하도록 구현 \\
\quad - 'local synchronous weight' variable 만들었음. (모든 thread들이 접근, 수정할 수 있는 weight) \\
\quad - 각자의 thread가 한 mini-batch를 처리(훈련) 하는데 update() -> record() ->map() 순서로 동작 \\ 
\quad pipeline scheduler에서 스케줄링 큐에 들어온 파티션의 backward 연산을 할 때 thread-safe인 상황이므로, local weight management method 들을 모두 backward 연산 마지막 부분에서 실행하게 되어 모든 thread가 공유하는 local synchronous weight를 안전하게  수정할 수 있다. \\
\\
\item method \\
\quad (1) update() \\
\quad - mini-batch를 처리하면서 계산된 gradient에 $\frac{1}{\LB+1}$ 곱해준다. \\
\quad (2) record() \\
\quad - 각 thread가 mini-batch를 처리하면서 계산된 gradient에 $\frac{1}{\LB+1}$ 곱한 값을 local synchronous weight에 업데이트 한다. \\
\quad (3) map() \\
\quad - 업데이트 된 local synchronous weight를 thread 자신이 연산하는 weight에 mapping.\\ 
\quad - 이러한 동작 흐름을 통해 이전 mini-batch들을 처리하면서 나온 gradient가 반영된 local synchronous weight를 이용하여 각 스레드는 새로운 mini-batch를 처리하게 됨으로서 아래와 같은 설명이 가능해진다. \\
\quad - For an $i$-th wave where $i \geq 1$, the weight used for a $j$-th minibatch
in the wave where $1 \leq j \leq \LB+1$ is compuated as follows:
\[ w_{i \times (\LB+1) + j} =  w_{i \times (\LB+1)} + \frac{1}{\LB+1} \times \sum_{k=1}^{j} u_{(i-1) \times (\LB+1)+k} \]
Note that 0-th wave composed of minibatches from 1 to $\LB+1$ uses $w_0$.
The system enforces that the last minibatch in a wave uses the weight including
all the updates from the previous wave.
\end{itemize}
\begin{itemize}
\item global weight management
\end{itemize}
(TODO: global 부분 동작 더 읽기): 1. the parameter server maintains the global clock  which is the minimum clock value among the local clock values of all the virtual workers. -> 1) 파라미터 서버가 모든 virtual worker의 clock을 가지고 있다. (모든 virtual worker의 clock을 variable에 (the number of virtual worker x 1) 행렬형태의 variable을 가지고 있다.) 2) inc\_vw\_clock(v): virtual worker v가 push 할때마다 해당 virtual worker의 clock을 증가시킨다.  3) min 연산을 통해 minimum clock value를 얻게 된다.
2.  Even while a faster {\VW} waits for a slower {\VW} to make a certain progress so that the faster {\VW} can get the global parameter within the {\GS} bound, the faster {\VW} may continue the execution for some minibatches, which have already started in the pipeline, if the {\LS} bound is not violated. -> async\_pull(): global parameter를 받기 위한(pull) 새로운 thread를 생성한다. mini-batch를 처리하는 virtual worker내의 thread들은 global staleness가 violate하기 전까지 pull에 상관없이 진행할 수 있다. global staleness를 violate하지 않는 last proceed step을 계산하여, 이보다 더 진행하려는 thread들을 block   시킨다. }
